MuRAL: A Multi-Resident Ambient Sensor Dataset Annotated with Natural Language for Activities of Daily Living

Recent progress in Large Language Models (LLMs) has enabled advanced reasoning and zero-shot recognition for human activity understanding with ambient sensor data. However, widely used multi-resident datasets such as CASAS, ARAS, and MARBLE lack natural language context and fine-grained annotation, limiting the full exploitation of LLM capabilities in realistic smart environments. To address this gap, we present MuRAL (Multi-Resident Ambient sensor dataset with natural Language), comprising over 21 hours of multi-user sensor data from 21 sessions in a smart home. MuRAL uniquely features detailed natural language descriptions, explicit resident identities, and rich activity labels, all situated in complex, dynamic, multi-resident scenarios. We benchmark state-of-the-art LLMs on MuRAL for three core tasks: subject assignment, action description, and activity classification. Results show that current LLMs still face major challenges on MuRAL, especially in maintaining accurate resident assignment over long sequences, generating precise action descriptions, and effectively integrating context for activity prediction. The dataset is publicly available at: https://mural.imag.fr/.

==> Tables/F1_scores.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\caption{Results of activity recognition of each class in different scenarios}
\label{tab: f1_score}
 \resizebox{\textwidth}{!}{
\begin{tabular}{|cc|cccc|cccc|cccc|}
\hline
\multicolumn{2}{|c|}{Metric}                                         & \multicolumn{4}{c|}{Precision (\%)}                                                                        & \multicolumn{4}{c|}{Recall (\%)}                                                                           & \multicolumn{4}{c|}{F1-score (\%)}                                                                         \\ \hline
\multicolumn{2}{|c|}{Scenario}                                       & \multicolumn{1}{c|}{Single\_A} & \multicolumn{1}{c|}{Multi\_A} & \multicolumn{1}{c|}{Single\_B} & Multi\_B & \multicolumn{1}{c|}{Single\_A} & \multicolumn{1}{c|}{Multi\_A} & \multicolumn{1}{c|}{Single\_B} & Multi\_B & \multicolumn{1}{c|}{Single\_A} & \multicolumn{1}{c|}{Multi\_A} & \multicolumn{1}{c|}{Single\_B} & Multi\_B \\ \hline
\multicolumn{1}{|c|}{\multirow{15}{*}{Class}} & Preparing Breakfast  & \multicolumn{1}{c|}{59.95}     & \multicolumn{1}{c|}{66.54}    & \multicolumn{1}{c|}{67.41}     & 80.07    & \multicolumn{1}{c|}{50.45}     & \multicolumn{1}{c|}{62.17}    & \multicolumn{1}{c|}{98.12}     & 84.38    & \multicolumn{1}{c|}{54.79}     & \multicolumn{1}{c|}{64.28}    & \multicolumn{1}{c|}{79.92}     & 82.16    \\
\multicolumn{1}{|c|}{}                        & Having Breakfast     & \multicolumn{1}{c|}{65.05}     & \multicolumn{1}{c|}{97.70}    & \multicolumn{1}{c|}{97.29}     & 96.20    & \multicolumn{1}{c|}{39.21}     & \multicolumn{1}{c|}{74.18}    & \multicolumn{1}{c|}{53.93}     & 82.05    & \multicolumn{1}{c|}{48.92}     & \multicolumn{1}{c|}{84.33}    & \multicolumn{1}{c|}{69.40}     & 88.56    \\
\multicolumn{1}{|c|}{}                        & Preparing Lunch      & \multicolumn{1}{c|}{25.08}     & \multicolumn{1}{c|}{27.37}    & \multicolumn{1}{c|}{67.31}     & 73.46    & \multicolumn{1}{c|}{30.02}     & \multicolumn{1}{c|}{17.84}    & \multicolumn{1}{c|}{100.}       & 68.74    & \multicolumn{1}{c|}{27.33}     & \multicolumn{1}{c|}{21.60}    & \multicolumn{1}{c|}{80.46}     & 71.02    \\
\multicolumn{1}{|c|}{}                        & Having Lunch         & \multicolumn{1}{c|}{5.19}      & \multicolumn{1}{c|}{47.87}    & \multicolumn{1}{c|}{100.}       & 47.78    & \multicolumn{1}{c|}{9.00}      & \multicolumn{1}{c|}{33.33}    & \multicolumn{1}{c|}{62.22}     & 66.23    & \multicolumn{1}{c|}{6.58}      & \multicolumn{1}{c|}{39.30}    & \multicolumn{1}{c|}{76.71}     & 55.51    \\
\multicolumn{1}{|c|}{}                        & Preparing Dinner     & \multicolumn{1}{c|}{21.53}     & \multicolumn{1}{c|}{64.90}    & \multicolumn{1}{c|}{66.22}     & 54.56    & \multicolumn{1}{c|}{73.84}     & \multicolumn{1}{c|}{84.78}    & \multicolumn{1}{c|}{67.59}     & 76.56    & \multicolumn{1}{c|}{33.33}     & \multicolumn{1}{c|}{73.52}    & \multicolumn{1}{c|}{66.90}     & 63.71    \\
\multicolumn{1}{|c|}{}                        & Having Dinner        & \multicolumn{1}{c|}{7.59}      & \multicolumn{1}{c|}{58.92}    & \multicolumn{1}{c|}{11.67}     & 31.39    & \multicolumn{1}{c|}{82.47}     & \multicolumn{1}{c|}{65.67}    & \multicolumn{1}{c|}{70.04}     & 29.91    & \multicolumn{1}{c|}{13.89}     & \multicolumn{1}{c|}{62.11}    & \multicolumn{1}{c|}{20.01}     & 30.63    \\
\multicolumn{1}{|c|}{}                        & Washing Dishes       & \multicolumn{1}{c|}{46.22}     & \multicolumn{1}{c|}{41.06}    & \multicolumn{1}{c|}{3.85}      & 10.37    & \multicolumn{1}{c|}{33.02}     & \multicolumn{1}{c|}{12.57}    & \multicolumn{1}{c|}{57.55}     & 7.97     & \multicolumn{1}{c|}{38.52}     & \multicolumn{1}{c|}{19.25}    & \multicolumn{1}{c|}{7.21}      & 9.00     \\
\multicolumn{1}{|c|}{}                        & Having Snack         & \multicolumn{1}{c|}{40.53}     & \multicolumn{1}{c|}{48.07}    & \multicolumn{1}{c|}{0.58}      & 12.84    & \multicolumn{1}{c|}{22.04}     & \multicolumn{1}{c|}{26.27}    & \multicolumn{1}{c|}{1.54}      & 44.42    & \multicolumn{1}{c|}{28.56}     & \multicolumn{1}{c|}{33.97}    & \multicolumn{1}{c|}{0.85}      & 19.92    \\
\multicolumn{1}{|c|}{}                        & Sleeping             & \multicolumn{1}{c|}{87.84}     & \multicolumn{1}{c|}{95.53}    & \multicolumn{1}{c|}{93.80}     & 97.84    & \multicolumn{1}{c|}{93.99}     & \multicolumn{1}{c|}{88.20}    & \multicolumn{1}{c|}{100}       & 97.82    & \multicolumn{1}{c|}{90.81}     & \multicolumn{1}{c|}{91.72}    & \multicolumn{1}{c|}{96.80}     & 97.83    \\
\multicolumn{1}{|c|}{}                        & Entertainment        & \multicolumn{1}{c|}{70.44}     & \multicolumn{1}{c|}{69.31}    & \multicolumn{1}{c|}{98.58}     & 89.45    & \multicolumn{1}{c|}{88.65}     & \multicolumn{1}{c|}{90.66}    & \multicolumn{1}{c|}{90.85}     & 90.28    & \multicolumn{1}{c|}{78.50}     & \multicolumn{1}{c|}{78.56}    & \multicolumn{1}{c|}{94.55}     & 89.86    \\
\multicolumn{1}{|c|}{}                        & Having Shower        & \multicolumn{1}{c|}{72.95}     & \multicolumn{1}{c|}{59.39}    & \multicolumn{1}{c|}{100}       & 60.27    & \multicolumn{1}{c|}{91.82}     & \multicolumn{1}{c|}{81.05}    & \multicolumn{1}{c|}{84.99}     & 86.57    & \multicolumn{1}{c|}{81.30}     & \multicolumn{1}{c|}{68.55}    & \multicolumn{1}{c|}{91.89}     & 71.06    \\
\multicolumn{1}{|c|}{}                        & Toileting            & \multicolumn{1}{c|}{82.67}     & \multicolumn{1}{c|}{53.74}    & \multicolumn{1}{c|}{82.40}     & 91.37    & \multicolumn{1}{c|}{76.86}     & \multicolumn{1}{c|}{81.43}    & \multicolumn{1}{c|}{96.76}     & 84.27    & \multicolumn{1}{c|}{79.66}     & \multicolumn{1}{c|}{64.75}    & \multicolumn{1}{c|}{89.00}     & 87.68    \\
\multicolumn{1}{|c|}{}                        & Working              & \multicolumn{1}{c|}{76.60}     & \multicolumn{1}{c|}{81.50}    & \multicolumn{1}{c|}{99.51}     & 98.39    & \multicolumn{1}{c|}{61.08}     & \multicolumn{1}{c|}{60.49}    & \multicolumn{1}{c|}{98.81}     & 85.63    & \multicolumn{1}{c|}{67.96}     & \multicolumn{1}{c|}{69.44}    & \multicolumn{1}{c|}{99.16}     & 91.57    \\
\multicolumn{1}{|c|}{}                        & Shaving              & \multicolumn{1}{c|}{/}         & \multicolumn{1}{c|}{84.16}    & \multicolumn{1}{c|}{/}         & 0.        & \multicolumn{1}{c|}{/}         & \multicolumn{1}{c|}{53.17}    & \multicolumn{1}{c|}{/}         & 0.       & \multicolumn{1}{c|}{/}         & \multicolumn{1}{c|}{65.17}    & \multicolumn{1}{c|}{/}         & 0.        \\
\multicolumn{1}{|c|}{}                        & Brushing Teeth       & \multicolumn{1}{c|}{75.24}     & \multicolumn{1}{c|}{46.63}    & \multicolumn{1}{c|}{1.09}      & 84.32    & \multicolumn{1}{c|}{43.86}     & \multicolumn{1}{c|}{34.30}    & \multicolumn{1}{c|}{0.40}      & 51.15    & \multicolumn{1}{c|}{55.42}     & \multicolumn{1}{c|}{39.53}    & \multicolumn{1}{c|}{0.58}      & 63.68    \\
\multicolumn{1}{|l|}{}                        & Talking on the Phone & \multicolumn{1}{c|}{98.67}     & \multicolumn{1}{c|}{42.83}    & \multicolumn{1}{c|}{/}         & 0.        & \multicolumn{1}{c|}{29.56}     & \multicolumn{1}{c|}{33.96}    & \multicolumn{1}{c|}{/}         & 0.        & \multicolumn{1}{c|}{45.49}     & \multicolumn{1}{c|}{37.88}    & \multicolumn{1}{c|}{/}         & 0.        \\
\multicolumn{1}{|l|}{}                        & Changing Clothes     & \multicolumn{1}{c|}{49.93}     & \multicolumn{1}{c|}{64.54}    & \multicolumn{1}{c|}{83.07}     & 95.19    & \multicolumn{1}{c|}{52.56}     & \multicolumn{1}{c|}{59.45}    & \multicolumn{1}{c|}{92.06}     & 82.95    & \multicolumn{1}{c|}{51.22}     & \multicolumn{1}{c|}{61.89}    & \multicolumn{1}{c|}{87.34}     & 88.65    \\ \hline
\multicolumn{2}{|c|}{Macro-Average}                                  & \multicolumn{1}{c|}{55.34}     & \multicolumn{1}{c|}{61.77}    & \multicolumn{1}{c|}{64.85}          & 60.20    & \multicolumn{1}{c|}{54.90}     & \multicolumn{1}{c|}{56.44}    & \multicolumn{1}{c|}{71.66}          & 61.11    & \multicolumn{1}{c|}{50.14}     & \multicolumn{1}{c|}{57.40}    & \multicolumn{1}{c|}{64.05}          & 59.46    \\ \hline
\multicolumn{2}{|c|}{Weighted-Average}                                  & \multicolumn{1}{c|}{66.00}     & \multicolumn{1}{c|}{77.67}    & \multicolumn{1}{c|}{92.37}     & 93.60    & \multicolumn{1}{c|}{67.56}     & \multicolumn{1}{c|}{76.23}    & \multicolumn{1}{c|}{93.79}     & 90.28    & \multicolumn{1}{c|}{76.95}     & \multicolumn{1}{c|}{86.49}    & \multicolumn{1}{c|}{93.08}     & 91.91    \\ \hline
\end{tabular}}
\end{table*}

==> Tables/sensor_error_rate.tex <==
\begin{table}[t]
\centering
\caption{Comparison of sensor error rate of two houses}
\label{tab: sensor_error}
\begin{tabular}{cccc}
\hline
House & Hours & \# Error Events & Error Rate \\ \hline
A     & 77.68          & 2834     & 36.48/hour               \\
B     & 279.31         & 0        & 0                     \\ \hline
\end{tabular}
\end{table}

==> Tables/table_comparison.tex <==
\begin{table}[t]
\centering
\caption{Comparison of performance between our method and the state of the art}
\label{tab:comparison}
% \setlength{\tabcolsep}{12pt}
\begin{tabular}{l|cccc}
\hline
Method & Resolution & Precision & Recall & F1-score \\ \hline
Gao et al.\cite{gao2024unsupervised}     & 5 minutes  & 96.00 & 95.56 & 95.60                    \\ 
LAHAR     & Second   & 88.54 & 92.31 & 90.39               \\
\hline
\end{tabular}
\end{table}

==> Tables/table_statistic.tex <==
\begin{table*}[t]
\centering
\caption{Statistics of the MuRAL Dataset.}
\label{tab: statistic}
  \resizebox{0.7\textwidth}{!}{  
\begin{tabular}{c|cccccccc}
\hline
\multirow{2}{*}{Session} & \multirow{2}{*}{\#Users} & \multirow{2}{*}{\#Events} & \multirow{2}{*}{\#Sensors} & \multirow{2}{*}{\#Description} & Description & \multirow{2}{*}{\#Activity} & \#Types of & Duration per   \\
                         &                          &                           &                            &                                & Length      &                             & Activity   & Activity (min) \\ \hline
mean                     & 3.00                     & 406.81                    & 18.76                      & 200.33                         & 11.67       & 41.71                       & 15.71      & 3.75           \\
std                      & 0.31                     & 72.86                     & 2.18                       & 53.57                          & 0.67        & 10.96                       & 2.21       & 1.35           \\
min                      & 2                        & 266                       & 15                         & 128                            & 9.84        & 20                          & 10         & 1.98           \\
max                      & 4                        & 558                       & 22                         & 284                            & 13.22       & 63                          & 19         & 7.01           \\ \hline
% 01                       & 3                        & 394                       & 21                         & 260                            & \textbf{9.84}        & \textbf{63}                          & \textbf{19}         & \textbf{1.98}           \\
% 02                       & 3                        & 518                       & 21                         & 283                            & 11.27       & 45                          & 17         & 3.75           \\
% 03                       & 3                        & 455                       & 20                         & 258                            & 11.40       & 59                          & 17         & 2.41           \\
% 04                       & 3                        & 450                       & 21                         & 255                            & 11.98       & 36                          & 18         & 2.94           \\
% 05                       & \textbf{4}                        & 349                       & 18                         & 188                            & \textbf{13.22}       & 58                          & 17         & 3.52           \\
% 06                       & \textbf{2}                        & 296                       & \textbf{15}                         & \textbf{128}                            & 11.49       & 32                          & 15         & 2.09           \\
% 07                       & 3                        & 351                       & 21                         & 243                            & 11.65       & 48                          & 15         & 2.64           \\
% 08                       & 3                        & 452                       & 16                         & 169                            & 11.93       & 50                          & 15         & 3.08           \\
% 09                       & 3                        & 456                       & 21                         & \textbf{284}                            & 11.76       & 45                          & 18         & 3.97           \\
% 10                       & 3                        & \textbf{266}                       & 16                         & 143                            & 11.85       & 30                          & 15         & \textbf{7.01}           \\
% 11                       & 3                        & 333                       & 18                         & 157                            & 11.48       & 45                          & 18         & 3.36           \\
% 12                       & 3                        & 338                       & 21                         & 216                            & 12.06       & 36                          & 14         & 5.08           \\
% 13                       & 3                        & 417                       & 18                         & 239                            & 11.10       & 55                          & 17         & 2.72           \\
% 14                       & 3                        & 430                       & 16                         & 132                            & 11.10       & 42                          & 13         & 4.03           \\
% 15                       & 3                        & 484                       & 20                         & 264                            & 12.37       & 45                          & 18         & 2.93           \\
% 16                       & 3                        & 361                       & \textbf{22}                         & 213                            & 11.66       & 35                          & 14         & 3.93           \\
% 17                       & 3                        & 444                       & 20                         & 169                            & 10.84       & 31                          & 17         & 4.26           \\
% 18                       & 3                        & 368                       & 18                         & 190                            & 12.38       & 38                          & 15         & 3.71           \\
% 19                       & 3                        & 471                       & 19                         & 137                            & 11.29       & 35                          & 16         & 2.94           \\
% 20                       & 3                        & \textbf{558}                       & 16                         & 133                            & 12.43       & 28                          & 12         & 5.56           \\
% 21                       & 3                        & 352                       & 16                         & 146                            & 11.89       & \textbf{20}                          & \textbf{10}         & 6.84           \\ \hline
\end{tabular}}
\end{table*}
